The Road Ahead for Networking: A Survey on ICN-IP Coexistence Solutions

In recent years, the current Internet has experienced an unexpected paradigm shift in the usage model, which has pushed researchers towards the design of the Information-Centric Networking (ICN) paradigm as a possible replacement of the existing architecture. Even though both Academia and Industry have investigated the feasibility and effectiveness of ICN, achieving the complete replacement of the Internet Protocol (IP) is a challenging task. Some research groups have already addressed the coexistence by designing their own architectures, but none of those is the final solution to move towards the future Internet considering the unaltered state of the networking. To design such architecture, the research community needs now a comprehensive overview of the existing solutions that have so far addressed the coexistence. The purpose of this paper is to reach this goal by providing the first comprehensive survey and classification of the coexistence architectures according to their features (i.e., deployment approach, deployment scenarios, addressed coexistence requirements and architecture or technology used) and evaluation parameters (i.e., challenges emerging during the deployment and the runtime behaviour of an architecture). We believe that this paper will finally fill the gap required for moving towards the design of the final coexistence architecture.

==> ICN_Overview_Advantages.tex <==
%hi
\iffalse
ih as das da s
\fi

==> icn.tex <==


\section{Internet of Today}

Existing Internet architecture was indeed designed three decades ago to inter-connect various heterogeneous networks. Moreover, the core of existing Internet is the TCP/IP protocol suite, which is used to interconnect network devices by putting protocols, applications and network channels together, and arranging them in four fundamental abstraction layers: Application, Transport, Link and Internet. This design leads to an hourglass shape with IP as the network layer as its “thin waist” \cite{ Akhshabi:2011:ELP:2018436.2018460}.

We consider IP which is used to enable Internet functionality to be as generic reference point when discussing possible coexistence of ICN and existing IP-based architectures. In particular, IP is in charge for routing packets from the source IP interface to its destination correspondingly. A host in IP, possibly have one or more IP interfaces, whereas a router has at least two. Moreover, to each IP interface there is at least one distinct fixed-length IP address for its indentation. The essential component of existing Internet architecture which subject to our analysis are IP based applications and services, transport protocols, DNS and CDNs. 

\subsection{Applications and services}
The existing Internet is full of IP based applications and services, utilizing the novel  capabilities of several protocols defined over the packet level IP service. The application layer is the platform where applications produce user data and transfer it to other applications on  other(s) of same host(s). The applications or services utilize the services provided by underlying layers, particularly Transport layer which delivers reliable or unreliable services to the processes. 

Among many higher level protocols, HTTP provides a conjunction point for these services with numerous web development frameworks based on the semantics provided by the hypertext transfer protocol. In recent years, even the services providing the multimedia data delivery have been migrating from the traditional RTP-over-UDP delivery to the various HTTP-level streaming solutions, e.g., DASH and others. To this end HTTP (and  even non HTTP) based requires considerations when migrating form existing IP-based architecture to ICN-based one. 

\subsection{Transport}

Applications use the Transport layer which establishes basic data channels and utilize them for  task-specific data exchange.  In particular, the layer maintains host-to-host connectivity by providing end-to-end message transfer which is independent of data structure, underlying network and the logistics of exchanging information for any particular explicit purpose.   The protocols in this layer are responsible to provide application addressing, segmentation and, error, congestion and flow control. The  fundamental categorization of end-to-end delivery is connection-oriented, applied in TCP, or connection-less, applied in UDP.




\subsection{Domain Name System}
The functionality of DNS is to translate the domain names (e.g., URL prefixes) into IP addresses. In particular, these names follows a hierarchical style where a upper level domain, e.g., \textit{.com} is tailed by various sub-level domains such as \textit{project.com} and   \textit{spritz.project.com}. An authoritative server is responsible to store, then  replies to the queries for an explicit contiguous portion of the domain name space, named as DNS zone. In addition, to increase DNS scalability, the authoritative name servers  are also capable to pass authority over sub-domains to further name servers. 

A user initially generates a DNS query to a local resolver, i.e., the process functioning on the user’s device which forwards the query to  the suitable name server(s). For this purpose, the resolver directs a UDP packet towards the DNS server, which is generally positioned in the resolver’s local network. The server first checks its local cache, and if not able to satisfy the query, it gets the appropriates reply from other or remote DNS servers.

Even though DNS was formerly designed with the purpose of static distributed database,  nowadays it also permits dynamic records updates and zone handovers.  Similarly, the work in proposed DNS as distributed database which also stores IP related information. For instance, [] proposed to store IPsec keys associated  data in DNS records and mapp them to IP addresses. 

\subsection{Content Delivery Networks}

Content Delivery Networks (CDN) are one of the utmost vital components of  today’s Internet. They were projected to maximize bandwidth, improve accessibility, and maintain correctness through content replication and bringing the content as close as possible to the hosts \cite{ 1250586}. The marketable accomplishment of the Internet and e-services, together with the exploding use of complex media content online has paved the way for the birth and growing interest in these networks. With CDNs, web content is distributed to cache servers located close to users, resulting in fast, reliable applications and Web services for the users. CDNs maintain multiple Points of Presence (PoP) with clusters of (the so-called surrogate) servers that store copies of identical content, such that users’ requests are satisfied by the most appropriate site. There are two general approaches to building CDNs. One is overlay model, which replicate content to thousands of servers worldwide. Another approach is network model which deploys code to routers and switches so that they can recognize specific application types and make forward decisions on the basis of predefined policies. Conventional CDNs can be mainly classified into two sub-categories, Commercial CDNs, and Academic CDNs.


\section{ICN Overview}\todo{DO IT}

The ICN concept was initially proposed in TRIAD \cite{Cheriton00triad:a},
which proposed name-based information communication. Since then, researchers
have proposed multiple architectures. In 2006, the data-oriented network
architecture (DONA) project \cite{Koponen:2007:DNA:1282380.1282402} at UC Berkeley proposed an ICN architecture,
which improved the security and architecture of TRIAD. The Publish Subscribe
Internet Technology (PURSUIT) \cite{6231280} project, a continuation of the Publish
Subscribe Internet Routing Paradigm (PSIRP) \cite{Dimitrov:2010:PPP:1839379.1839409} project, both funded by the EU
Framework 7 Program (FP7), have proposed a publish/subscribe protocol stack that
replaces the IP protocol stack. In another approach, the Network of Information
(NetInf) project \cite{Dannewitz:2013:NII:2459510.2459643} was initially proposed by the European FP7 4WARD \cite{4ward}. project, and further development has been made by the Scalable and Adaptive
Internet Solutions (SAIL) \cite{sail} project. Similarly, Van Jacobson, a Research Fellow
at PARC, proposed the Content Centric Networking (CCN) project \cite{Jacobson} in 2007.
Currently work is being performed to enhance the CCN architecture called
“named-data networks” (NDN) \cite{Zhang}.

The core idea behind information-centric networking (ICN) architectures is that
who is communicating is less significant than what data are required. This paradigm
shift has occurred due to end-users’ use of today’s Internet, which is more
content-centric than location-centric, e.g., file sharing, social networking, or
retrieval of aggregated data. 
The ICN approach fundamentally decouples information from its sources, by means of a clear location-identity split. The basic assumption behind this is that information is named, addressed, and matched independently of its location, therefore it may be located anywhere in the network \cite{ Arianfar:2010:CRD:1921233.1921240, Diallo2011LeveragingCF}. In ICN, instead of specifying a source-destination host pair for communication, a piece of information itself is named. An indirect implication (and benefit) of moving from the host naming model to the information naming model, is that information retrieval becomes receiver-driven. In contrast to the current Internet where senders have absolute control over the data exchanged, in ICN no data can be received unless it is explicitly requested by the receiver. In ICN, after a request is sent, the network is responsible for locating the best source that can provide the desired information. Routing of information requests thus seeks to find the best source for the information, based on a location-independent name.



Although ICN architectures are still under active development, all these 
architectures address a set of key functionalities, albeit with
different approaches. Below we illustrate key functionalities \cite{6563278}, which are the basis for presenting and analyzing
the various ICN initiatives. 

\subsection{Naming}
The structure of the name assigned to a piece of information (or service) that can be communicated over the network is one of the main characteristics of each ICN architectural proposal. In all ICN architectures information names are location-independent. On the other hand, depending on the approach, names may range from flat to hierarchical and may or may not be human-readable. 
\subsection{Name resolution and Data routing}
 Name resolution involves matching an information name to a provider or source that can supply that information, while data routing involves constructing a path for transferring the information from that provider to the requesting host. There are  two approaches for these functions, i.e.,  integrated, or coupled, or are independent, or decoupled. In the coupled approach, the information request is routed to an information provider, which subsequently sends the information to the requesting host by following the reverse path over which the request was forwarded. In the decoupled approach, the name resolution function does not determine or restrict the path that the data will use from the provider to the subscriber. For example, an independent data routing module may send to the provider a source route to the requesting host.
 
 
\subsection{Caching}
ICN architectures provides two variant of caching, i.e.,  on-path and off-path caching. In on-path caching the network exploits information cached along the path taken by a name resolution request, while in off-path caching the network exploits information cached outside that path. In ICN architectures with decoupled name resolution and data routing, off-path caching is supported by the name resolution system, which handles caches as regular information publishers. In case, name resolution and data transfer are coupled, off-path caching is supported by the routing system used to forward the requests for information.

\subsection{Mobility}

Subscriber mobility is intrinsically supported in ICN architectures, since mobile subscribers can just send new subscriptions for information after a handoff. Publisher mobility is more difficult to support, since the name resolution system (in the coupled approach) or the routing tables (in the decoupled approach) need to be updated. Several proposals for handling producer mobility exist in ICN literature~\cite{7562050,Anastasiades2014}.

\subsection{Security}
 
In contrast to IP, where security is provided by the upper layers to secure host-to-host communication, ICN comes with security in mind. In ICN, the content is explicitly shared along with the signature key of the producer, which is used to verify the integrity of the received content. In particular, security in ICN follows a data-centric model. Therefore, the content is signed by the content provider, allowing interest senders to verify its integrity and data-origin authentication~\cite{Compagno2018}.
